Multilingual CheckList: Generation and Evaluation

Multilingual evaluation benchmarks usually contain limited high-resource languages and do not test models for specific linguistic capabilities. CheckList is a template-based evaluation approach that tests models for specific capabilities. The CheckList template creation process requires native speakers, posing a challenge in scaling to hundreds of languages. In this work, we explore multiple approaches to generate Multilingual CheckLists. We device an algorithm - Template Extraction Algorithm (TEA) for automatically extracting target language CheckList templates from machine translated instances of a source language templates. We compare the TEA CheckLists with CheckLists created with different levels of human intervention. We further introduce metrics along the dimensions of cost, diversity, utility, and correctness to compare the CheckLists. We thoroughly analyze different approaches to creating CheckLists in Hindi. Furthermore, we experiment with 9 more different languages. We find that TEA followed by human verification is ideal for scaling Checklist-based evaluation to multiple languages while TEA gives a good estimates of model performance.

==> archive/2_checklist_overview.tex <==
\section{CheckList Overview}\label{sec:checklist-overview}

CheckList \citep{checklist-paper} is a behavioral testing approach for evaluation of NLP systems. In this approach, first we need to identify a set of {\em capabilities} (linguistic nuances) required to solve the underlying ``task'', and create set of templates that test them individually.
%It begins with the identification of capabilities and creation of a set of templates that test those capabilities. The linguistic nuances that the model claiming to solve a ``task'' must handle are known as {\em capabilities}. 
For example, Negation is a capability that is essential to model for Sentiment Analysis task; the model should be able to distinguish `happy' and `not happy' as two opposite sentiments. The {\em templates}, in turn, are used to alongwith keywords and its corresponding lexicon to generate the final test-suite.

For example, if \texttt{\{CITY\} is \{ADJ\}} is a template, for which \texttt{CITY} and \texttt{ADJ} are the keywords, and their corresponding lexicons are \texttt{CITY=[Delhi, Paris, New York] } and \texttt{ADJ=[wonderful, beautiful, nice, famous]}. From this template and lexicon, various test examples can be generated such as \texttt{Paris is wonderful} and \texttt{New York is famous}. Models are tested on these generated examples to assess their various capabilities.  
%%%%% Do we need this? #Somak: commenting out
% Checklist also allows a keyword to be used multiple times in a template by appending a cardinal to it, e.g., 
% \textbf{T0}: \texttt{\{CITY-0\} is bigger than \{CITY-1\}}. 
% In this case, both the placeholders will be populated with the values of the keyword \texttt{CITY}. There is a separate signal (remove\_duplicates flag) which indicates whether both the values can be same or not.
%%%%% Do we need this? #Somak: commenting out
%(if the remove\_duplicates flag is True, the examples generated would not have any example where the value of \texttt{CITY-0} and \texttt{CITY-1} is same, otherwise such examples will exist). 
Additionally, CheckList uses 3 different types of tests namely Minimum Functionality (MFT), Invariance (INV) and Directionality (DIR) tests. MFT is the equivalent of unit tests in software engineering. For INV and DIR test, pre-existent test-cases are perturbed in such a way that the labels are expected to change (or remain the same for INV) in a specific manner. In this work we focus only on MFTs. 

==> archive/amcg-s.tex <==
\section{Automated Multilingual Checklist Generation (AMCG)}\label{sec:amcg}

\begin{figure*}[t]
\centering
\includegraphics[scale=0.4]{Images/amcg_algo1.png}
\caption{AMCG Algorithm with lexicon candidate selection}\label{fig:amcg_algo}
\end{figure*}

Due to word order and other syntactic differences between languages, a word-for-word or any other heuristic methods for translation of templates do not seem feasible. Due to similar reasons, extraction of target template from translation of a single sentence generated from the source template is not reliable either. In fact, different sentences generated from a source template might have very different structures when translated into the target language due to natural variation in translation, stochasticity in the MT models, and also syntactic divergence (for instance, in agreement rules) between the languages. 

On the other hand, using the target translations of all or a large number of test-cases generated from the source sentences is also suboptimal because of the following reasons. First, it does not qualify as a target CheckList; it is just a test-set, at best. Second, such a set is costly or impossible to verify by a human, as one has to go through every test-case separately; instead, a manual CheckList creation in the target language from scratch or manual translation of source templates would be much less effort-intensive. Third, the quality of such a test-set will strongly depend on the quality of the MT system.

We propose an Automated CheckList generation approach, AMCG, that mitigates the aforementioned problems, yet retaining the benefits of the extreme approaches. AMCG induces the target templates from the translation of a large number of test-cases generated from a source template. By doing so, on one hand it is able to appropriately handle syntactic divergence through splitting/merging of templates as required; on the other hand, it is able to tolerate noise and variation in translations by learning from a large set of translations. 


\subsection{Notations and Conventions}
\label{sec:convention}

A template can be considered as a type of grammar to generate sentences where the keywords are the non-terminals and their corresponding lexicons are the terminal symbols. While the templates generate a finite set of sentences (representing a {\em Regular Language}), %they represent a {\em Regular language} (and hence a {\em Context Free language}). However, 
the individual templates might be context-sensitive. Consider the template T0 ``\texttt{CITY-0} is beautiful but \texttt{CITY-1} is bigger.'' Here,  \texttt{CITY-1} should be different than \texttt{CITY-0}; and hence the non-terminal symbols cannot be replaced independently of each other. Therefore, we cannot use existing methods such as (probabilistic) context free grammar induction to learn templates from sentences.  %introduced above.
%\begin{quote}
%    T0: \texttt{CITY-0} is beautiful but \texttt{CITY-1} is bigger.\\
%    \texttt{CITY} =  \{Delhi, Paris, New York\} ,
%\end{quote}
% \begin{align*}
%     \text{T}:~ & ~\text{\texttt{CITY-0} is beautiful but \texttt{CITY-1} is bigger.} \\ 
%     \texttt{CITY} & =  \{\text{New York, Paris, Delhi}\} , 
% \end{align*}
 %we can not replace \texttt{CITY-1} by its corresponding terminal symbols without looking what terminal symbol is used for \texttt{CITY-0} and vice versa and hence it is not a context free grammar. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Our Convention for Templates}\label{sec:convention}

% In this work we follow a slightly different notion of templates that are more convenient in generating multilingual checklist.  Every set of sentences that can be generated using the original templates described by \cite{checklist-paper}, can be generated using the our template(s) as well. Our convention is described below

 We use {\em terminal} and {\em non-terminal} to denote {\em lexicons} and {\em keywords} respectively. In a template, if the non-terminals are appended with cardinals from 0 to $k$, then they can \emph{not} be replaced with same terminal while generating sentences. Also, if a template contains an instance of a non-terminal with cardinal $k, (k>0)$ then at least one instance of the same non-terminal with cardinal $k-1$ should have occurred before its occurrence in the template. 



\subsection{The AMCG Algorithm}
Figure \ref{fig:pipeline} shows the pipeline of the entire AMCG process. Without loss of generality, we assume that En is the source language and Hi is the target language. We start with an En template and corresponding terminals created by a human expert, and generate a set of examples by substituting the non-terminals with their appropriate terminals. We then translate the examples to Hi using an MT system - Azure cloud Translator for this study. Then, our proposed AMCG algorithm first extracts a potential set of terminals by grouping words and assign them a symbol/name (non-terminals). In the second step, we extract the Hi templates using the terminals and non-terminals. %Then we extract Hi template(s), terminal(s) and non-terminal(s) from the Hi examples. 
The entire pipeline of extracting Hi templates are repeated for each of the En templates, resulting in a (tentative) CheckList for Hi. 
 
%Our proposed AMCG algorithm extracts Hi templates (along with Hi terminal words) from the Hi examples. First we discuss our approach to extract potential set of terminal words, i.e., we group a set of words (terminals) and give them a symbol/name (non-terminal). Then we extract the templates using the terminals and non-terminals that are extracted in the previous step. %We also discuss scalability challenges and ways to address them. 

\subsection{Extracting and Grouping Terminals}\label{sec:find_lexicon}

First, we convert the given Hi examples into a directed graph whose nodes are unique words (or tokens) from the examples and there is an edge from word A to word B if word B follows word A in at least one of the examples. In this directed graph (as shown in Fig.~\ref{fig:amcg_algo}), between any two nodes, if there are multiple paths of length less than equal to $k+1$ (we set $k$ to 2), we concatenate the intermediate words in the path (with space in between them) and treat them as terminals. This set of terminals, between the two nodes, are grouped together represented by a non-terminal symbol (for example Key\_1 and Key\_2 in Fig.~\ref{fig:amcg_algo}). 


 
\subsection{Template Extraction given Terminal and Non-Terminals}\label{sec:extract_template}

Input to our algorithm is (1) a set Hi examples, $S = \{s_1, s_2, \ldots s_N \}$, and (2) all non-terminals $v_i = {w_{i1}, w_{i2}, \ldots}$, where $w_{ij}$ are terminals (obtained in the previous step). In other words, these are the production rules from a non-terminal to (only) terminals. Output of the algorithm is a set of templates $\hat{T} = \{t_1, t_2, ...\} $ such that $\hat{T}$ can generate all the examples in $S$ using only the given non-terminal and their corresponding terminals. %We represent non-terminals and its corresponding terminals as a list (or ordered set) of tuples $L = [\langle w_1, v_1 \rangle... \langle w_i, v_i \rangle ... ] $. The tuple $\langle w_i, v_i \rangle$ belongs to $L$ if and only if the the terminal $w_i$ corresponds to the non-terminal $v_i$. 

A trivial construction of $\hat{T}$ is $S$ itself, as $S$ can generate every example. However, we would like to find the (approximately) smallest $\hat{T}$ such that it can generate entire $S$. 
To this end, we develop the AMCG algorithm (outlined in Algorithm~\ref{alg:extract_template}), which we explain next. 
First, for each sentence $s_i$, we call the function \textsc{Get-Templates-Per-Example} to generate a set of templates, $T_i = \{t_{i1}, t_{i2}, ...\}$, such that $s_i$ belongs to the set of examples generated by each $t_{ij}$. %(refer Lemma \ref{lemma1}). 
Moreover, every possible template that can generates $s_i$, using only the given terminals and non-terminal, belongs to $T_i$.  %(refer Lemma \ref{lemma2}). 
Once we have $T_i$ for every $s_i$, we construct the (approximately) smallest set $\hat{T}$ such that $\forall i, \hat{T} \bigcap T_i \neq \emptyset $. Note that for every sentence $s_i \in S$, there exist atleast one template in $\hat{T}$ that generates $s_i$. % -- refer lemma \ref{lemma3}. 
Finding the smallest $\hat{T}$ (refer lemma \ref{lemma4}) is a variant of set cover problem, and we use a greedy approximation algorithm. %to find an approximate solution.  

% \begin{lemma}\label{lemma1}
% Every template $t_{ik} \in T_i$ generates the sentence $s_i$
% \end{lemma}

% \begin{lemma}\label{lemma2}
% Every template that generates $s_i$ using only the given terminals and non-terminals, is present in $T_i$
% \end{lemma}

% \begin{lemma} \label{lemma3}
% Set $\hat{T}$ can generate every sentences in $S$
% \end{lemma}

\begin{lemma}\label{lemma4}
If a set $\hat{T}$ is the smallest set such that $\forall i, \hat{T} \bigcap T_i \neq \emptyset $, then $\hat{T}$ is the smallest set that generates every sentence in $S$ using only the given terminals and non-terminals. 
\end{lemma}

Proof of the Lemma %\ref{lemma1}, \ref{lemma2}, \ref{lemma3} and 
\ref{lemma4} are in appendix. 


\paragraph{Generating $T_i$ per Example} For every terminal string ($w_m$) that is a substring of an example $s_i$, we have 2 options while creating a  template, either (1) replace the matched substring ($w_m$) with its corresponding non-terminal ($v_m$) or (2) leave as it is. We can make this decision independently for every matched terminal. However, we need to carefully assign the cardinals for repeating non-terminals and make sure the templates conform to the adopted convention mentioned in \S \ref{sec:convention}. We use the functions \textsc{Replace-Matched-String} and \textsc{Rename-Nonterminal-cardinals} to ensure such conformance. The \textsc{Replace-Matched-String}  function replaces the matched terminal $w_{m}$ in $t_{ij}$ with its corresponding non-terminal $v_{m}$. For multiple $w_{m}$ in $t_{ij}$, each $w_{m}$ is either retained or replaced indepently of the rest. \textsc{Rename-Nonterminal-cardinals} renames the cardinals to make sure that an instance of non-terminal with cardinal $k-1$ occurs before the instance of a non-terminal with cardinal $k, (k>0)$.


% \paragraph{\textsc{Replace-Matched-String}} \label{sec:Replace-Matched-String}
% This function replaces the matched terminal $w_{m}$ in $t_{ij}$ with its corresponding non-terminal $v_{m}$. If there are multiple $w_{m}$ in $t_{ij}$, then each $w_{m}$ will be independently replaced with $v_{m}$ or left unchanged. For example, say the initial template and $\langle$terminal, non-terminal$\rangle$ pair are ``\#Paris is beautiful. \texttt{CITY-0} is cold. Paris is bigger.'' and $\langle$Paris, \texttt{CITY}$\rangle$ respectively. This will generate 3 templates after replacement. 
% (1) "\#\texttt{CITY-1} is beautiful. \texttt{CITY-0} is cold. Paris is bigger." 
% (2) "\#Paris is beautiful. \texttt{CITY-0} is cold. \texttt{CITY-1} is bigger." 
% (3) "\#\texttt{CITY-1} is beautiful. \texttt{CITY-0} is cold. \texttt{CITY-1} is bigger." 

%Note that, we do not search if the words in the $s_i$ is a terminal, rather we search if the terminal is a sub-string of $s_i$ (or $t_{ij}$). This makes it possible to match for the terminal with a sub-word or a multi-word string. Sub-word match can be quite useful in the morphologically rich languages. %using only the base word as lexicons it maybe possible to match different morphological forms. 

% \paragraph{\textsc{Rename-Nonterminal-cardinals}} \label{sec:Rename-Nonterminal-cardinals}
% This functions renames the cardinals to make sure that an instance of non-terminal with cardinal $k-1$ occurs before the instance of that non-terminal with cardinal $k, (k>0)$. For example, after re-naming the cardinals, the above three templates become the following three, respectively. 
% (1) "\#\texttt{CITY-0} is beautiful. \texttt{CITY-1} is cold. Paris is bigger." 
% (2) "\#Paris is beautiful. \texttt{CITY-0} is cold. \texttt{CITY-1} is bigger." 
% (3) "\#\texttt{CITY-0} is beautiful. \texttt{CITY-1} is cold. \texttt{CITY-0} is bigger." 




\setlength{\textfloatsep}{0pt}
\begin{algorithm}[t]
\caption{Extract templates given terminals and non-terminals}\label{alg:extract_template}
\begin{algorithmic}[1]
\Require{$S = \{s_1, s_2, ....s_N \}$,  $L = [\langle w_1, v_1 \rangle... \langle w_i, v_i \rangle ... ]$ }
\Ensure{$\hat{T}$, the approximately smallest set of templates that generates entire $S$}
\For{each $s_i$ in S}
    \State $T_i \gets $ \Call{Get-Templates-Per-Example}{$s_i, L$}
\EndFor
\State Find (approximately) smallest $\hat{T}$ such that $\forall T_i,  \hat{T} \cap T_i \neq \emptyset$ \Comment{Variant of set cover, use greedy approach}
\State \textbf{return $\hat{T}$}

\Procedure{Get-Templates-Per-Example}{$s_i, L$}
\State $T_i  \gets \{s_i\}$
\For{each $\langle w_m, v_m \rangle$ in $L$}
    \State $T_{new} \gets \{\}$
    \For{each $t_{ij}$ in $T_i$ }
        \If{$w_m$ is sub-string of $t_{ij}$}
            \State $t_{new} \gets $ \Call{Replace-Matched-String}{$t_{ij}, w_m, v_m$} 
            \State $t_{new} \gets $ \Call{Rename-Nonterminal-cardinals}{$t_{new}$} 
            \State $T_{new} \gets T_{new} \cup t_{new} $
        \EndIf
    \EndFor 
    \State $T_i  \gets T_i \cup T_{new}$ 
\EndFor
\State \textbf{return} $T_i$
\EndProcedure
\end{algorithmic}
\end{algorithm}



\subsubsection{Combine both the steps}

First, we find all the potential terminals and non-terminals (using 
\S~\ref{sec:find_lexicon}) for all Hi examples, and then use them to extract template following the algorithm outlined in \S~\ref{sec:extract_template}. While this may generate correct templates, it is often computationally expensive. Primarily due to noise in translation (many of the translated sentences may not fit into a template), the algorithm to extract terminals and non-terminals (\S~\ref{sec:find_lexicon}) often gives a lot of different non-terminals that share many common terminals. For example we may get two non-terminals with their corresponding terminals such as ``\{Paris, New York, Delhi\}''  and  ``\{London, New York, Delhi\}''. Moreover, the complexity of algorithm in \S~\ref{alg:extract_template} to extract templates can increase exponentially with the number of non-terminals. To mitigate this problem, we follow an iterative approach where instead of using all the extracted non-terminals (along with their terminals), we initialize the set of non-terminals with an empty set and iteratively add the most useful non-terminals (with their corresponding terminals) to the existing set of non-terminals. Refer appendix section for further discussion. 

==> archive/amcg-short.tex <==
\section{Automated Multilingual Checklist Generation (AMCG)}\label{sec:amcg}

\begin{figure*}[t]
\centering
\includegraphics[scale=0.4]{Images/amcg_algo1.png}
\caption{AMCG Algorithm with lexicon candidate selection}\label{fig:amcg_algo}
\end{figure*}
% \begin{figure}[t]
% \centering
% \includegraphics[height=0.3\textheight]{Images/amcg_algo1_v2.png}
% \caption{AMCG Algorithm with lexicon candidate selection}\label{fig:amcg_algo}
% \end{figure}
We first describe our proposed method to automatically generate CheckList in a target language from a source language CheckList.

Due to syntactic differences between languages, heuristic approaches (including transliteration) for direct translation of templates is not feasible. Extraction of target template from translation of a single sentence generated from a source template is not reliable either, as target translations of different sentences generated from a source template might have different structures due to natural variation in translation, stochasticity of MT models, and syntactic divergence, for instance in agreement rules, between the languages. 

On the other hand, using the target translations of all or a subset of the test-cases generated from the source templates is also suboptimal because (1) it does not qualify as a target CheckList; it is just a test-set, at best; and (2) such a translated set is costly or impossible to verify by a human, as one has to go through every test-case individually; instead, a manual CheckList creation in the target language from scratch or manual translation of source templates would be more efficient. Moreover, the quality of such a test-set will strongly depend on the quality of the MT system.

We propose an Automated CheckList generation approach, AMCG, that mitigates the aforementioned problems by inducing the target templates from the translation of a large number of test-cases generated from a source template. By doing so, on one hand it is able to appropriately handle syntactic divergence through splitting/merging of templates as required; on the other hand, it is able to tolerate noise and variation in translations by learning from a large set of translations. 


\subsection{The AMCG Algorithm}
Figure \ref{fig:pipeline} shows the pipeline of the entire AMCG process. Without loss of generality, we assume that En is the source and Hi is the target language. We start with an En template and corresponding terminals created by a human expert, and generate a set of examples by substituting the non-terminals with their appropriate terminals. We then translate the examples to Hi using an MT system - Azure cloud Translator for this study. Then, our proposed AMCG algorithm first extracts a potential set of terminals by grouping words and assigning them a symbol/name (non-terminals). In the second step, we extract the Hi templates using the terminals and non-terminals. %Then we extract Hi template(s), terminal(s) and non-terminal(s) from the Hi examples. 
The entire pipeline of extracting Hi templates are repeated for each of the En templates, resulting in a (tentative) CheckList for Hi. AMCG has three steps, as described below. We provide the details, pseudocode and proofs in the Appendix.

\noindent
\textbf{Step 1: Group Terminals and Non-Terminals} First, we convert the Hi sentences generated from an En template into a directed graph whose nodes are unique words (or tokens) from the examples and there is an edge from word A to word B if word B follows word A in at least one of the examples. In this directed graph (as shown in Fig.~\ref{fig:amcg_algo}), between any two nodes, if there are multiple paths of length less than equal to $k+1$ (we set $k$ to 2), we concatenate the intermediate words in the path (with space in between them) and treat them as terminals. This set of terminals, between the two nodes, are grouped together represented by a non-terminal symbol (for example Key\_1 and Key\_2 in Fig.~\ref{fig:amcg_algo}).

% \setlength{\textfloatsep}{0pt}
% \begin{algorithm}[t]
% \caption{Extract templates given terminals and non-terminals}\label{alg:extract_template}
% \begin{algorithmic}[1]
% \Require{$S = \{s_1, s_2, ....s_N \}$,  $L = [\langle w_1, v_1 \rangle... \langle w_i, v_i \rangle ... ]$ }
% \Ensure{$\hat{T}$, the approximately smallest set of templates that generates entire $S$}
% \For{each $s_i$ in S}
%     \State $T_i \gets $ \Call{Get-Templates-Per-Example}{$s_i, L$}
% \EndFor
% \State Find (approximately) smallest $\hat{T}$ such that $\forall T_i,  \hat{T} \cap T_i \neq \emptyset$ \Comment{Variant of set cover, use greedy approach}
% \State \textbf{return $\hat{T}$}
% \end{algorithmic}
% \end{algorithm}
\noindent
\textbf{Step 2: Template Extraction} Using a set of Hi sentences, $S = \{s_1, s_2, \ldots s_N \}$, and all non-terminals $v_i = {w_{i1}, w_{i2}, \ldots}$, where $w_{ij}$ are terminals (obtained in the previous step), our algorithm outputs a set of templates $\hat{T} = \{t_1, t_2, ...\} $ such that $\hat{T}$ can generate all the examples in $S$ using only the given non-terminal and their corresponding terminals. For each sentence $s_i$, we 
%call the function \textsc{Get-Templates-Per-Example} to 
generate a set of candidate templates, $T_i = \{t_{i1}, t_{i2}, ...\}$, such that $s_i$ belongs to the set of examples generated by each $t_{ij}$. Finding the smallest $\hat{T}$ is a variant of set cover problem, and we use a greedy approximation algorithm.

%\begin{lemma}\label{lemma4}
%If a set $\hat{T}$ is the smallest set such that $\forall i, \hat{T} \bigcap T_i \neq \emptyset $, then $\hat{T}$ is the smallest set that generates every sentence in $S$ using only the given terminals and non-terminals. 
%\end{lemma}

\noindent
\textbf{Step 3: Combine Both Steps} The above template extraction process, while resulting in correct outputs, may be computationally expensive due to translation noise\footnote{For example, many of the translated sentences may not fit into a template. The algorithm may produce a set of  distinct non-terminals that share many common terminals. For example, we may get two non-terminals with their corresponding terminals such as ``\{Paris, New York, Delhi\}''  and  ``\{London, New York, Delhi\}''.} and its time-complexity that is exponential on the number of non-terminals.   To mitigate this problem, we follow an iterative approach where instead of using all the extracted non-terminals (along with their terminals), we initialize the set of non-terminals with an empty set and iteratively add the most useful non-terminals (with their corresponding terminals) to the existing set of non-terminals. 

==> archive/extra.tex <==

% Moreover, comparison of the generated tests sets from this paradigm is complicated and has multiple facets. To this end, we propose metrics to evaluate the checklists generated on measures of soundness, diversity, and resourcefulness (\S \ref{sec:metrics}). We provide a detailed discussion of the  results (\S \ref{sec:results}), the lesons learnt during the process (\S \ref{sec:discussion}), and also note various challenges in multilingual checklist generation (\S \ref{sec:challenges}).



% Our main contribution is the introduction of Automated Multilingual Checklist Generation AMCG (\S \ref{sec:amcg}) to generate multilingual checkists with no human supervision. We also experiment with three more methods of multilingual checklist generation (\S \ref{sec:userstudy}). Two of these rely completely on native speakers while the third one is a human-in-loop technique where the checklist is created automatically and then verified and corrected by a native speaker. 



% Transformer-based language models have become a norm in NLP today. Further, their multilingual versions like XLM-Roberta \citep{xlmr} and mBERT \citep{bert} have the potential to scale NLP applications to about a hundred languages, many of them under-served and under-resourced, in a zero-shot setting. These models (and their derivatives) have a state-of-art performance on various cross-lingual transfer benchmarks and datasets such as XNLI \citep{xnli} or XGLUE \citep{xglue}.

% Despite impressive performance on standard benchmarks, NLP systems have been known to fail in real world settings. Models tend to learn spurious patterns to achieve high accuracies \citep{balanced_vqa_v2, gururangan-etal-2018-annotation, glockner2018breaking, tsuchiya2018performance, geva2019we}. There is also a risk of overestimation of performance due to similar train and test sets in static benchmarks \citep{belinkov2017synthetic, recht2019imagenet}. Moreover, the benchmarks don't evaluate models for language specific nuances that the model would be otherwise expected to cater to.

% To mitigate this and better understand what the models can and cannot do, non-standard evaluation techniques are gaining attention. Non-standard evaluation is an umbrella term that is used to refer to evaluating aspects including but not limited to robustness \citep{rychalska2019models}, fairness \citep{prabhakaran-etal-2019-perturbation}, consistency \citep{ribeiro-etal-2019-red}, explanations \citep{ribeiro2016why}, and adversarial performance \citep{ribeiro-etal-2018-semantically, iyyer2018adversarial, nie2020adversarial}. 

% Checklist \citep{checklist-paper} is recent non-standard evaluation paradigm that aims to evaluate black-box NLP systems through software-engineering like testing. The tests are designed based on linguistic capabilities that the NLP system would be expected to have. This evaluation revealed colossal failures in basic capabilities of state-of-art and commercial systems for three tasks. Further, the insights from a Checklist based evaluation can also be used to improve a system \citep{humaneval_eacl_case_study}. We describe Checklist in \S \ref{sec:checklist-overview}.

% However, most of these works focus on evaluating English systems. While Checklist provides limited multilingual support, it is not enough to allow seamless evaluation of multilingual system. In this work we systematically experiment porting an English Checklist to another language, specifically Hindi, for evaluating Sentiment Analysis and NLI. 



% Our main contribution is the introduction of Automated Multilingual Checklist Generation AMCG (\S \ref{sec:amcg}) to generate multilingual checkists with no human supervision. We also experiment with three more methods of multilingual checklist generation (\S \ref{sec:userstudy}). Two of these rely completely on native speakers while the third one is a human-in-loop technique where the checklist is created automatically and then verified and corrected by a native speaker. 

% Moreover, comparison of the generated tests sets from this paradigm is complicated and has multiple facets. To this end, we propose metrics to evaluate the checklists generated on measures of soundness, diversity, and resourcefulness (\S \ref{sec:metrics}). We provide a detailed discussion of the  results (\S \ref{sec:results}), the lesons learnt during the process (\S \ref{sec:discussion}), and also note various challenges in multilingual checklist generation (\S \ref{sec:challenges}).





% For example: `I \{neg\_verb\} \{activity\}.' is a template. `NEGATIVE\_VERB' and `ACTIVITY' in this template are two different keywords in the lexicon, each taking a specific set of values. For example, NEGATIVE\_VERB = [`hate', `dislike', `despise'] and ACTIVITY = [`cleaning', `cooking']. The template generates 6 examples. 

% SEC CHECKLIST

% Checklist \citep{checklist-paper} is a behavioral testing technique for evaluating NLP systems. They enable humans to easily create template sets and tests based on linguistic capabilities to test black-box NLP models in a decoupled software-engineering like fashion\footnote{\url{https://github.com/marcotcr/checklist}}. The authors show that state-of-the-art and commercial systems across three tasks revealing unprecedented failure rates even for the most basic capabilities.  

% The linguistic nuances that the model must handle are known as capabilities. For example, Negation is a capability of a Sentiment Analysis model - the model should be able to distinguish `happy' and `not happy' as two opposite sentiments despite the overlapping word `happy'. The capabilities form the basis of creating template sets and tests.

% In order for humans to generate test cases, Checklist uses Templates and Lexicons. For example: `I \{NEGATIVE\_VERB\} \{ACTIVITY\}.' is a template. `NEGATIVE\_VERB' and `ACTIVITY' in this template are two different keywords in the lexicon, each taking a specific set of values. For example, NEGATIVE\_VERB = [`hate', `dislike', `despise'] and ACTIVITY = [`cleaning', `cooking']. The template generates 6 examples - the Cartesian product of the values of the two lexicon keywords in the template.

% The examples from the template sets will results in tests. The Minimum Functionality Tests (MFTs) are equivalent of unit tests to test specific phenomena. The Invariance (INV) and Directionality (DIR) are test types where the model output is expected to not change and change respectively for specific pertubations in the test cases. In our work we focus only on MFTs.

% For more details we refer readers to \citet{checklist-paper}.



==> archive/morelangs.tex <==
\section{Experiments with Multiple Languages}

\begin{table*}
\centering
\begin{tabular}{llllllll} 
\toprule
\textbf{Language}                  & \textbf{Method} & \textbf{Vocabulary} & \textbf{Temporal} & \textbf{Fairness} & \textbf{Negation} & \textbf{SLR} & \textbf{Robustness}  \\ 
\hline
\textbf{English}                   & DES             & 24.21               & 1.8               & 94.35             & 48.16             & 35.94        & 42.58                \\ 
\hline
\multirow{2}{*}{\textbf{Hindi}}    & AMCG            & 43.04               & 16.43             & 87.65             & 53.98             & 41.78        & 48.77                \\
                                   & VER             & 29.68               & 12.37             & 88.3              & 62.84             & 42.94        & 52.25                \\ 
\hline
\multirow{2}{*}{\textbf{Gujarati}} & AMCG            & 39.12               & 34.97             & 87.46             & 51.84             & 47.37        & 52.09                \\
                                   & VER             & 29.09               & 32.18             & 88.72             & 55.14             & 46.8         & 51.54                \\ 
\hline
\multirow{2}{*}{\textbf{French}}   & AMCG            & 20.27               & 11.22             & 86.52             & 56.55             & 40.09        & 46.77                \\
                                   & VER             & 21.78               & 11.53             & 86.52             & 61.25             & 40.09        & 47.8                 \\ 
\hline
\multirow{2}{*}{\textbf{Swahili}}  & AMCG            & 46.04               & 37.5              & 88.86             & 73.32             & 51.87        & 58.45                \\
                                   & VER             &                     &                   &                   &                   &              &                      \\ 
\hline
\textbf{Arabic}                    & AMCG            & 47.83               & 14.1              & 91.57             & 47.69             & 39.97        & 52.58                \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparing AMCG on multiple languages: } We report the failure  of XLM-R model, finetuned on SST dataset, on examples generated using AMCG and VER. Failure rates of AMCG and VER are comparable}
\label{tab:difflangs}
\end{table*}

%Up to now, the entire discussion has been done with the Target language as Hindi. 
In order to ascertain that the algorithm works well for other languages as well, we conduct a study with 4 more languages other than English and Hindi. We choose French, Swahili, Arabic, and Gujarati as our language of choice because they are typologically diverse and also are at varied points in the resource spectrum. 
%French is High-resource while Swahili is very low-resourced. Hindi itself can be considered a mid-resourced language. Gujarati has good similarity to Hindi, but comparatively lower resources. Arabic lies somewhere in the middle of French and Hindi on the resource spectrum. 
We used a subset of templates from the original checklist for sentiment analysis and create multilingual checklists using the AMCG algorithm. The results for different languages can be seen in Table \ref{tab:difflangs}. All results are obtained on a XLMR model finetuned with SST
% with the same hyper parameters as that of the Roberta model original checklist paper.

Some known patterns are seen in these results. English has the lowest failure rates as expected for all but Fairness. French, being high-resources has the second lowest failure rates in most cases. Swahili on the other hand, being very low-resourced has the highest failure rates. The trend of AMCG results on Fairness seems to have a reverse trend, and it is unclear as to why that is the case. Among Hindi and Gujarati, which are similar languages, Gujarati has higher failure rates than Hindi, which is again expected since Gujarati is lower-resourced compared to Hindi. Yet another known trend since is the exceptionally high failure rate of Negation in Swahili. Previous work has also shown that LMs dont handle Negation in Swahili very well due to the morphological/linguistic peculiarity of the way in which negation is done in Swahili. We then asked annotators (native or near native proficient speakers) of Hindi, Gujarati, French, and Swahili to correct the templates generated by AMCG. Results on this corrected template are also in the table \ref{tab:difflangs}. These results present optimistic findings. For all the languages, the failure rates before and after correction by a human are very similar. This means that even without any human resource, the failure rates induced by un-corrected AMCG templates can provide a good estimate of how well the model is doing for particular capabilities in different languages. The only capability where this did not remain true was vocabulary. We observed that this was most likely because of literal translations. For examples a sentence - 'the service was poor' gets translated to 'vah seva gareeb hai'. here gareeb in Hindi is the translation of poor, but the translation is literal, in the sense that gareeb means 'economically poor'. Hence, the translation fails to reflect the original meaning of the sentence which does not use poor in the literal sense, but in a more implicit form referring to 'bad'. There are many such literal translations like 'lame' getting translated to 'langda' which is a literal translation as the word langda refers to a 'one legged person'. Due to such examples it is likely that the failure rate of uncorrected AMCG template are higher. However, when human correction happens, such terminals that don't make sense for the context are removed by the annotator and hence the failure rates decrease. Overall however, we can say that for most cases, AMCG would be a good estimator to the performance of the system even if no human resources are used to verify the templates it generates.

